Revisiting the Classics: On the Statistics of Dust Formation in Novae

While nova eruptions produce some of the most common and dramatic dust formation episodes among astrophysical transients, the demographics of dust-forming novae remain poorly understood. Here, we present a statistical study of dust formation in 40 novae with high-quality optical/IR light curves, quantitatively distinguishing dust-forming from non-dust-forming novae while exploring the properties of the dust events. We find that 50-70% of novae produce dust, significantly higher than previous estimates. Dust-forming novae can be separated from those that do not show dust formation by using the largest redward ($V-K$) colour change from peak visible brightness; ($V-J$) or ($V-H$) offer useful but less sensitive constraints. This makes optical+IR photometry a powerful tool to quantify dust formation in novae. We find that novae detected in GeV $\gamma$-rays by \emph{Fermi}-LAT appear to form dust more often than novae not detected by \emph{Fermi}, implying a possible connection between $\gamma$-ray producing shocks and dust production. We also find that novae that evolve very quickly ($t_2 < 10$ days) are much less likely to form dust, in agreement with previous findings. We confirm a correlation between $t_2$ and the time of the onset of dust formation (which occurs $\sim$1 week--3 months after maximum light), but conclude that it is primarily an observational artifact driven by dust formation determining when a nova drops 2 mag below peak. The significant fraction of novae that form dust make them ideal laboratories in our Galactic backyard to tackle the puzzle of dust formation around explosive transients.

==> Makefile <==
#
# ---=== Ultimate LaTeX astronomy paper/proposal makefile ===---
#
# Run 'make' to compile a LaTeX source and display the reulting PDF with 'okular'
# The Makefile understands 'latex'/'pdflatex' with or without 'bibtex'.
# The Makefile will apply a set of tests aiming to catch common typos, repeated words, 
# check US/British spelling and some aspects of AAS/MNRAS journal style.
#
# The Makefile assumes it is run by GNUmake and relies on external tools including cat, cut, grep, sed, awk, and okular
# 
# The originla version of this Makefile was created by Kirill Sokolovsky <kirx@kirx.net>
#
######################################################################################################
# Manual setttings that modify the makefile behaviour

# Set to "yes" if this is an arXiv sumbission (needs .bbl file) otherwise set "no" (remove .bbl file on cleanup)
ARXIV=no
#ARXIV=yes

# Display the compiled document using okular or other PDF viewer? (yes/no)
LAUNCH_PDF_VIEWER_TO_DISPLAY_COMPILED_PAPER=yes

# is texcount is not installed the Makefile will complain about it but will not fail
COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT=yes

# make a grayscale copy of the PDF - think of the colorblind people and the ones with cheap laser printers
PRODUCE_BLACK_AND_WHITE_COPY_OF_THE_PDF_TO_CHECK_HOW_IT_LOOKS=no

# Disable some individual tests if needed (yes -- test enabled / no -- test disabled)
#
# demand \textsc{MyCodeName}
TEST_SOFTWARE_TEXTSC=no
CODE_NAMES_CASE_INSENSITIVE := IRAF MIDAS AIPS CASA DS9 XSPEC HEASoft Fermitools Difmap DiFx PIMA SExtractor PSFEx PyZOGY lightkurve photutils
CODE_NAMES_CASE_SENSITIVE := VaST

# warn about UTF8 characters in the .tex source files
TEST_NONASCII_CHARS=yes
# do not allow km/s, demand km\,s^{-1} instead
TEST_KM_S=no

######################################################################################################
# Automated setup: try hard to find the main tex file and recognize its format: PDF figure, BibTeX...
#

# manually exclude some tex filenames from consideration
ALL_TEXFILES_FOR_GRAMMAR_CHECK := $(shell ls *.tex | grep -v -e 'aassymbols.tex' -e '_backup' -e '_BACKUP' -e '_BASE' -e '_LOCAL' -e '_REMOTE')

# Set *main.tex as the main TeX file, otherwise assume the largest TeX file is the main TeX file
TEXFILE_BASENAME := $(shell if [ -f *main.tex ];then ls *main.tex ;else ls -S $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) ;fi | head -n1 | sed 's:.tex::g')


PDFTEX := $(shell cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -e 'includegr' -e 'file' | grep --quiet -e '.pdf' -e '.png' && echo 'yes' )
BIBTEX := $(shell cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet 'bibliographystyle' && echo 'yes' )

BIBFILENAME := $(shell cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep 'bibliography{' | head -n1 | awk -F'bibliography{' '{print $$2}' | awk -F'}' '{print $$1".bib"}')

MODIFY_BIBFILE_ULTRACOMPACT_REF := $(shell cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet -e 'bibliographystyle.mnras_shortlisthack' -e 'bibliographystyle.supershort_numbers_oneline' && echo 'yes' )

MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING := $(shell cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep 'documentclass' | grep --quiet 'mnras' && echo 'yes' )

AAS_MANUSCRIPT_REQUIRING_US_SPELLING := $(shell cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep 'documentclass' | grep --quiet -e 'aastex' -e 'emulateapj' && echo 'yes' )

# if somehow both MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING and AAS_MANUSCRIPT_REQUIRING_US_SPELLING are set to 'yes'
# set MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING to 'no' and prefer the US spelling
ifeq ($(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING),yes)
ifeq ($(AAS_MANUSCRIPT_REQUIRING_US_SPELLING),yes)
MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING := no
endif
endif

# First, case-insensitive and then case-sensitive search for names of common astronomy codes
ANY_KNOWN_SOFTWARE_MENTIONED := $(shell \
    for code in $(CODE_NAMES_CASE_INSENSITIVE); do \
        if cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g' | sed 's/\\citep{[^}]*}//g' | sed 's/\\cite{[^}]*}//g' | sed 's/\\citealt{[^}]*}//g' | sed 's/\\texttt{[^}]*}//g' | grep --quiet --ignore-case -e "\\b$$code\\b" ; then \
            echo 'yes'; \
            exit; \
        fi; \
    done; \
    for code in $(CODE_NAMES_CASE_SENSITIVE); do \
        if cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g' |  sed 's/\\citep{[^}]*}//g' | sed 's/\\cite{[^}]*}//g' | sed 's/\\citealt{[^}]*}//g' | sed 's/\\texttt{[^}]*}//g' | grep --quiet -e "\\b$$code\\b" ; then \
            echo 'yes'; \
            exit; \
        fi; \
    done)


IS_SWIFT_UVOT_MENTIONED := $(shell cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet -e 'Swift' && cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet -e 'UVOT' && echo 'yes' )


all: info clean check_utf8 check_spell check_robot_words check_no_whitespace check_coma_instead_of_period check_extra_white_space try_to_find_duplicate_words shorten_journal_names_bib check_british_spelling check_us_spelling check_gamma_ray_math_mode check_software_small_capitals check_swift_uvot_lowercase_filternames check_km_s check_units check_consistent_unbreakable_space_size_UT check_consistent_Halpha_Hbeta check_consistent_multiwavelength check_phrasing check_filenames_good_for_arXiv  $(TEXFILE_BASENAME).pdf  produce_balck_and_white_copy_of_the_pdf check_for_bonus_figures  display_compiled_pdf


info: $(TEXFILE_BASENAME).tex
	@echo "Starting the ultimate LaTeX Makefile"
	@echo "TEXFILE_BASENAME= "$(TEXFILE_BASENAME)
ifeq ($(BIBTEX),yes)
	@echo "BIBFILENAME= "$(BIBFILENAME)
else
	@echo "No BibTeX, fine"
endif

clean: 
ifeq ($(ARXIV),yes)
	# do not remove .bbl file for arXiv submission
	rm -f $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~ $(TEXFILE_BASENAME)_grayscale.pdf
else
	# remove .bbl file and everything else
	rm -f $(TEXFILE_BASENAME).bbl  $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~ $(TEXFILE_BASENAME)_grayscale.pdf
endif


check_utf8: $(TEXFILE_BASENAME).tex
ifeq ($(TEST_NONASCII_CHARS),yes)
	#
	# Display any non-ASCII UTF8 characters higlighting them with color.
	# (If this check fails, but you see no color in the output -
	# the non-ASCII character is masquerading as white space and
	# you may need to select text with mouse to see the offending character.)
	#
	@echo "Searching for non-ASCII characters in TeX file"
	{ LC_ALL=C grep --color=always '[^ -~]\+' $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) && exit 1 || true; }
	#{ LC_ALL=C grep --color=always '[^ -~]\+' $(TEXFILE_BASENAME).tex && exit 1 || true; }
	# Check that the TeX file type is not Unicode - but that may miss some stray Unicode character
	file $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep -e 'Unicode' -e 'ISO-8859' && exit 1 || true; }
	#file $(TEXFILE_BASENAME).tex | { grep Unicode && exit 1 || true; }
ifeq ($(BIBTEX),yes)
	@echo "Searching for non-ASCII characters in BibTeX file"
	{ LC_ALL=C grep --color=always '[^ -~]\+' $(BIBFILENAME) && echo 'WARNING: Unicode character in .bib file - trying to fix' && cp $(BIBFILENAME) $(BIBFILENAME).backup && sed -i 's/\(\x09\|\x0B\|\x0C\|\xC2\xA0\|\xE2\x80\x80\|\xE2\x80\x81\|\xE2\x80\x82\|\xE2\x80\x83\|\xE2\x80\x84\|\xE2\x80\x85\|\xE2\x80\x86\|\xE2\x80\x87\|\xE2\x80\x88\|\xE2\x80\x89\|\xE2\x80\x8A\|\xE2\x80\xAF\|\xE2\x81\x9F\|\xE3\x80\x80\|\x98\)/ /g'  $(BIBFILENAME) || true; }
	{ LC_ALL=C grep --color=always '[^ -~]\+' $(BIBFILENAME) && echo 'ERROR: Unicode character in .bib file' && exit 1 || true; }
endif
endif


check_spell: $(TEXFILE_BASENAME).tex
	# Case-insensitive search
	# sed 's/[^ ]*.eps[^ ]*//ig'   is to make sure figure filenames are ignored
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:the A config::g' | sed 's:a-priori::g' | sed 's:a priori::g' | sed 's:binary tree::g' | sed 's:pile up::g' | sed 's:pile~up::g' | sed 's/[^ ]*.eps[^ ]*//ig' | sed 's/\\url{[^}]*}//g' | { grep --color=always --ignore-case -e 'compliment' -e 'complimented' -e 'ile up' -e 'ile~up' -e '\bcan will\b' -e '\bmay can\b' -e '\bmay will\b' -e '\ba the\b' -e '\bthe a\b' -e '\bwhited\b' -e '\bneutrons star\b' -e '\bhotpot\b' -e '\brang\b' -e 'has be seen' -e 'synchroton' -e '\bhight\b' -e 'far from being settled' -e 'recourses' -e '\bwile\b' -e 'will allows' -e '\btree\b' -e '\ban new\b' && exit 1 || true; }
	# Case-sensitive search
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:the A config::g' | { grep --color=always -e 'x-ray' -e ' tp ' && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -ie 's/\\[A-Za-z0-9]* / /g' | { grep --color=always 'countrate' && echo "SHOULD BE count rate" && exit 1 || true; }
	# Use \b to match on "word boundaries", which will make your search match on whole words only.
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always '\bgenue\b' && echo "SHOULD BE genuine" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always '\bTHe\b' && echo "SHOULD BE the" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'maid' && echo "DID YOU MEAN made ?" && exit 1 || true; }
	# 'substraction' is a rare synonym for 'embezzlement' https://www.merriam-webster.com/dictionary/substraction
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'substraction' && echo "DID YOU MEAN subtraction ?" && exit 1 || true; }
	# and the all-time classic
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'redshit' && echo "DID YOU MEAN redshift ?" && exit 1 || true; }
	# 'common-envelop' is not your ordinary package for a letter
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bcommon-envelop\b' && echo "DID YOU MEAN common-envelope ?" && exit 1 || true; }
	# ' on Fig'
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bon Fig' && echo "DID YOU MEAN in Fig... ?" && exit 1 || true; }
	#
	# 'number if'
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bnumber if\b' && echo "DID YOU MEAN number of ?" && exit 1 || true; }
	# novae instead of novas, unless it looks like software name 'NOVAS' - a popular astrometry library
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -e 's/textsc{[^{}]*}//g' | sed -e 's/texttt{[^{}]*}//g' | sed -e 's/url{[^{}]*}//g' | { grep --color=always '\bnovas\b' && echo "DID YOU MEAN novae ?" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bloosing\b' && echo "DID YOU MEAN losing ? othewise use loosening" && exit 1 || true; }
	# Appending~\ref{
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e '\bAppending~\\ref{' -e '\bAppending \\ref{' && echo "DID YOU MEAN Appendix~\\ref{" && exit 1 || true; }
	# GHz
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always -e '\bGHZ\b' -e '\bGhz\b' && echo "SHOULD BE  GHz" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'tune able' && echo "SHOULD BE tunable" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'thejet' && echo "SHOULD BE the jet" && exit 1 || true; }

check_robot_words:  $(TEXFILE_BASENAME).tex
	# Words and phrases normal people do not use
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bdelve\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bgrappling\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bunleash\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\btestament\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bjourney\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bsupercharge\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bembrace\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bburning question\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bunlock\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\buplevel\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\brevolutionize\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bgroundbreaking\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\belevate\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bin the wake of\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\bavid\b' && echo "ARE YOU A ROBOT?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'It is important to note' && echo "DON'T WRITE LIKE THAT IF YOU ARE A HUMAN" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e "I can't help with that" -e "Is there something else I can help you with" -e "I'm not able to fulfill" -e "That's not something I can do" -e "I can offer assistance on a wide range of topics" -e "I can't proceed with this specific request" -e "I'm sorry but as a AI language model" -e "Here are some" && echo "ARE YOU KIDDING ME?" && exit 1 || true; }
	
check_no_whitespace: $(TEXFILE_BASENAME).tex
	#  cut -f1 -d"%" -- ignore everything after %
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	#
	# period      sed 's:[A-Z].[A-Z].::g' will allow for two capital letter combinations like initials K.S.
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:R.A.::g' | sed 's:L.A.Cosmic::g' | sed 's:\\.M::g' | sed 's:Obs.ID::g' | sed 's:U.S.::g' | sed 's:H.E.S.S.::g' | sed 's:J.D.L.::g' | sed 's:K.V.S.::g' | sed 's:E.A.::g' | sed 's:Ras.Pi::g' | sed 's:Ph.D.::g' | sed 's:P.O.::g' | sed 's:[A-Z].[A-Z].[A-Z].::g'  | sed 's:[A-Z].[A-Z].::g' | { grep --color=always -e '\.[A-Z]' && exit 1 || true; }
	# two periods
	# sed -e 's/\.\.\.//g' -- allow for three periods 
	# sed -e 's/\.\.\///g' -- allow for '../' as in file path
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\.\.\.//g' | sed -e 's/\.\.\///g' | { grep --color=always -e '\.\.' && exit 1 || true; }
	# coma periods;   sed 's:\\,::g' -- remove unbreakable half-spaces from the test
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e '\,\.' && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e ',\.' && exit 1 || true; }
	# some journal styles allow ".," combination: "e.g.,"
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\.\,' && exit 1 || true; }
	# two comas;   sed 's:\\,::g' -- remove unbreakable half-spaces from the test
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e '\,\,' && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:\\,::g' | { grep --color=always -e ',,' && exit 1 || true; }
	# missing \ref (but allow \href {http://...} and stuff like {dblp:#1})
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | grep -v -e 'href ' -e ':#1}' | { grep --color=always -E -e '~{\w*:' -e ' {\w*:' && echo "MISSING \\ref{} ?" && exit 1 || true; }
	# White space between Fig. and ref
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Fig \\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figs \\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Fig\, \\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figs\. \\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Fig\.\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figs\.\\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Fig\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figs\\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Fig~\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figs~\\ref' && echo "SHOULD BE Figs.~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figure\\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figures\\ref' && echo "SHOULD BE Figures~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figure \\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always 'Figures \\ref' && echo "SHOULD BE Figures~\\ref{}" && exit 1 || true; }
	# White space before \cite
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:\\protect\\citeauthoryear::g' | sed 's:\\protect\\citename::g' | { grep --color=always '[a-z]\\cite' && echo "NO WHITE SPACE BEFORE \\cite" && exit 1 || true; }

check_extra_white_space: $(TEXFILE_BASENAME).tex
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v -e '\.\.\/' -e ' \.\/' | { grep --color=always ' \.' && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always ' \,' && exit 1 || true; }

check_coma_instead_of_period: $(TEXFILE_BASENAME).tex
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | grep -v -e 'Uni' -e 'Obs' -e 'Inst' -e 'The Netherlands' -e 'The United' | { grep --color=always -e '\,The' -e '\, The' && exit 1 || true; }

check_units: $(TEXFILE_BASENAME).tex
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always '\bhr\b' && echo "SHOULD BE h ACCORDING TO IAU RECOMMENDATIONS ON UNITS https://www.iau.org/publications/proceedings_rules/units/" && exit 1 || true; }

check_phrasing: $(TEXFILE_BASENAME).tex
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\ballow one to identify\b' -e '\ballow to identify\b' && echo "SHOULD BE allow the identification of" && exit 1 || true; }

try_to_find_duplicate_words: $(TEXFILE_BASENAME).tex
	#
	# Checking for repeated words over linebreaks
	# We do not exclude comments, so line numbers will be correct
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	# grep -v ' \-\-[A-Za-z]'    -- remove command line arguments examples
	#                   ' & '    -- ignore tables that may well have duplicate words/numbers
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | grep -v -e ' \--[A-Za-z]' -e ' & ' | cut -f1 -d"%" | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	#  sed 's/%.*$//'    -- remove everything after %
	#  sed '/^[[:space:]]*$/d' -- remoove empty lines
	# The output line nubers may not be exact as we skip comment lines
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | grep -v -e ' \--[A-Za-z]' -e ' & ' | cut -f1 -d"%" | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	#
	# Catch word repeats in one line (obsolete)
	# The old version that doesn't catch everything
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	#cat $(TEXFILE_BASENAME).tex | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | grep -v -E '[0-9]cm' | grep -v -E '[0-9]in' | grep -v -e '&' -e 'textwidth' -e 'includegraphicx' -e 'includegraphics' -e 'tabular' | { egrep "(\b[a-zA-Z]+) \1\b"  && exit 1 || true; }
	# The new experimental version
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	# mess 'caption{}' and 'captionbox{}' as we still want to check for repeated words in captions
	# sed -n '/filecontents/,/filecontents/!p'  -- ignore everything between these lines (it's an embedded file)
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | grep -v -e ' \--' -e ' & ' | sed -n '/filecontents/,/filecontents/!p' | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ein --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	# Last-trench effort -- just grep for the most common repetitions
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always -e ' the the ' -e ' a the ' && exit 1 || true; }
	#
	#######################
	# sed 's/[[:blank:]]\+/ /g' - replace multiple white spaces with one white space
	# Search for suspicious word combinations
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always  "\bare know\b" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always -e "\bmission line\b" -e "\bmission lines\b" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always "\bwill be also be\b" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always "\bdivided my the\b" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always "\bthe on\b" && exit 1 || true; }
	# "the were" -> "they were"
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bthe were\b' && echo "DID YOU MEAN they were ?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bthe were\b' && echo "DID YOU MEAN they were ?" && exit 1 || true; }
	# "Through this paper" -> "Throughout this paper"
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bThrough this paper\b' && echo "DID YOU MEAN throughout this paper ?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bThrough this paper\b' && echo "DID YOU MEAN throughout this paper ?" && exit 1 || true; }
	# "in order to not" -> "in order not to"
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bin order to not\b' && echo "DID YOU MEAN in order not to ?" && exit 1 || true; }	
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bin order to not\b' && echo "DID YOU MEAN in order not to ?" && exit 1 || true; }	
	# two version -> two versions
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case -e '\btwo version\b' -e '\bthree version\b' -e '\bfour version\b' -e '\bfive version\b' -e '\bsix version\b' -e '\bseven version\b' -e '\beight version\b' -e '\bnine version\b' -e '\bten version\b' -e '\beleven version\b' -e '\btwleve version\b' && echo "DID YOU MEAN versions ?" && exit 1 || true; }	
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case -e '\btwo version\b' -e '\bthree version\b' -e '\bfour version\b' -e '\bfive version\b' -e '\bsix version\b' -e '\bseven version\b' -e '\beight version\b' -e '\bnine version\b' -e '\bten version\b' -e '\beleven version\b' -e '\btwleve version\b' && echo "DID YOU MEAN versions ?" && exit 1 || true; }	
	# minor and minor axes
	#cat *.tex | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case 'minor and minor axes' && echo "DID YOU MEAN major and minor axes ?" && exit 1 || true; }	
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case 'minor and minor axes' && echo "DID YOU MEAN major and minor axes ?" && exit 1 || true; }
	#
	# try to check the use of temporary (adjective) vs temporarily (adverb)
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\btemporary \(degrade\|improve\|decrease\|display\|create\|destroy\|add\|remove\|close\|open\|suppress\|promote\|express\|release\|capture\|stimulate\|enhance\|localize\|available\|unavailable\|excite\|calm\|dull\|relax\|accelerate\|decelerate\|withdraw\|trap\|recover\|confine\|free\|here\|there\|accessible\|inaccessible\|appear\|disappear\)\(d\|ed\)\?\b' && echo "CHECK the use of temporary (adjective) vs temporarily (adverb)" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bhole mas\b' && echo "DID YOU MEAN black hole mass ?" && exit 1 || true; }	
	# general an/and
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case -E '\b(an)\s+[bcdfgjklmpqstvwyz]' && echo "CHECK the use of an vs and  (test 1)" && exit 1 || true; }
	# an disappear
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\ban \(young\|include\|exclude\|degrade\|improve\|decrease\|display\|create\|destroy\|add\|remove\|close\|suppress\|promote\|express\|release\|capture\|stimulate\|enhance\|localize\|available\|unavailable\|excite\|calm\|dull\|relax\|accelerate\|decelerate\|withdraw\|trap\|recover\|confine\|free\|here\|there\|accessible\|inaccessible\|appear\|disappear\)\b' && echo "CHECK the use of an vs and  (test 2)" && exit 1 || true; }
	# last a few day
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\blast a few \(second\|minute\|hour\|day\|month\|year\)\b' && echo "CHECK last a few ...s" && exit 1 || true; }
	# is excludes
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bas is \(include\|exclude\|degrade\|improve\|increase\|decrease\|display\|create\|destroy\|add\|remove\|close\|open\|suppress\|promote\|express\|release\|capture\|stimulate\|enhance\|localize\|available\|unavailable\|excite\|calm\|dull\|relax\|accelerate\|decelerate\|withdraw\|trap\|recover\|confine\|free\|here\|there\|accessible\|inaccessible\|appear\|disappear\)\(s\|d\|ed\)\?\b' && echo "CHECK the use of is vs it" && exit 1 || true; }
	# these is no doubt
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bthese is no doubt\b' && echo "SHOULD BE there is no doubt" && exit 1 || true; }
	# further away
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bfurther away\b' && echo "SHOULD BE farther away" && exit 1 || true; }
	# further than
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bfurther than\b' && echo "SHOULD BE farther than" && exit 1 || true; }
	# out analysis
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bout analysis\b' && echo "SHOULD BE our analysis" && exit 1 || true; }
	# from at
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\bfrom at\b' && echo "SHOULD BE form at OR from OR at" && exit 1 || true; }
	# even grades
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | sed 's/[[:blank:]]\+/ /g' | { grep --color=always --ignore-case '\beven grades\b' && echo "SHOULD BE event grades" && exit 1 || true; }
	
	
# This hack will modify the .bib file replacing some long journal names if we are using mnras_shortlisthack.bst style
shorten_journal_names_bib: $(BIBFILENAME)
ifeq ($(MODIFY_BIBFILE_ULTRACOMPACT_REF),yes)
	# Modify .bib
	@echo "I WILL RUIN THE BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
	# If the bibfile looks unmodified, save a backup copy
	cat $(BIBFILENAME) | { grep -e '{ATel}' -e '{RNAAS}' -e '{AN}' || cp -v $(BIBFILENAME) $(BIBFILENAME)_backup_long_journal_names ; }
	# Do the actual modification
	cat $(BIBFILENAME) | sed 's:{The Astronomer.s Telegram}:{ATel}:g' | sed 's:{Research Notes of the American Astronomical Society}:{RNAAS}:g' | sed 's:{Astronomische Nachrichten}:{AN}:g' > $(BIBFILENAME)_tmp && mv -v $(BIBFILENAME)_tmp $(BIBFILENAME)
else
	# Nothing to do
	@echo "KEEP THE ORIGINAL BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
endif

check_british_spelling:
ifeq ($(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING),yes)
	# Check for British spelling
	# MNRAS style guide https://academic.oup.com/mnras/pages/General_Instructions#6%20Style%20guide
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE Acknowledgements (this is how the section is named in the MNRAS template)" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'timescale' && echo "SHOULD BE time-scale" && exit 1 || true; }
	# random collection of astronomy-specific words
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'barycenter' && echo "SHOULD BE barycentre" && exit 1 || true; }
	# random collection of words
	# sed 's/\\[^~]*{//g'  will remove \textcolor{
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\[^~]*{//g' | grep -v -e 'xcolor' -e 'rgbcolor' -e 'sec:' -e 'fig:' -e '.pdf}' | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'traveling' && echo "SHOULD BE travelling" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'behavior' && echo "SHOULD BE behaviour" && exit 1 || true; }
	# Use \b to match on "word boundaries", which will make your search match on whole words only.
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's:laborator::g' | sed 's:ollaboration::g' | grep -v '$^{' | { grep --color=always '\blabor\b' && echo "SHOULD BE labour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '\banalog\b' && echo "SHOULD BE analogue" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'centimeter' && echo "SHOULD BE centimetre" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	# Other MNRAS things
	# https://academic.oup.com/mnras/pages/general_instructions#6.5%20Miscellaneous%20journal%20style
	#cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always --ignore-case -e '\\%' -e 'percent' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | { grep --color=always '\\%' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\,' && echo "SHOULD BE e.g." && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\.\,' && echo "SHOULD BE i.e." && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case '``' && echo "SHOULD BE \`" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case "''" && echo "SHOULD BE \'" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'eq\.' -e 'eqn\.' -e 'Eq\.' -e 'Eqn\.' && echo "SHOULD BE equation~()" && exit 1 || true; }
else
	# Nothing to do
	@echo "THIS DOES NOT LOOK LIKE A MNRAS MANUSCRIPT - NOT ENFORCING BRITISH SPELLING"
	echo $(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING)
endif

check_us_spelling:
ifeq ($(AAS_MANUSCRIPT_REQUIRING_US_SPELLING),yes)
	# Check for US spelling
	# AAS style guide https://journals.aas.org/aas-style-guide/
	# they also suggest follow The Chicago Manual of Style https://www.chicagomanualofstyle.org/home.html
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centred' && echo "SHOULD BE centered" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centre' && echo "SHOULD BE center" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulphur' && echo "SHOULD BE sulfur" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'labelled' && echo "SHOULD BE labeled" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's:analyses::g' | sed 's:Analyses::g' | { grep --color=always --ignore-case 'analyse' && echo "SHOULD BE analyze / analyzed  see https://www.chicagomanualofstyle.org/book/ed17/part2/ch07/psec003.html" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrized' && echo "SHOULD BE parameterized" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrize' && echo "SHOULD BE parameterize" && exit 1 || true; }
	# Why I was under impression that 'acknowledgements' is the correct spelling in AAS journals?
	# Their style guide spells 'acknowledgments' https://journals.aas.org/manuscript-preparation/#acknowledgments
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE acknowledgements" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgements' && echo "SHOULD BE acknowledgments" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'artefact' && echo "SHOULD BE artifact" && exit 1 || true; }
	# Yes, best-fitting seems to be OK at AAS
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fitting ' && echo "SHOULD BE best-fit" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e ' disc\,' -e ' disc\.' -e 'disc$$' -e 'disc ' && echo "SHOULD BE disk" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'haloes' && echo "SHOULD BE halos" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case ' on to ' && echo "SHOULD BE onto" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'time-scale' -e 'time scale' -e 'time~scale' && echo "SHOULD BE timescale" && exit 1 || true; }
	#
	# random collection of words
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'colour' && echo "SHOULD BE color" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavour' && echo "SHOULD BE flavor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'humour' && echo "SHOULD BE humor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labor' && echo "SHOULD BE labour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labour' && echo "SHOULD BE labor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbour' && echo "SHOULD BE neighbor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyse' && echo "SHOULD BE paralyze" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalogue' && echo "SHOULD BE catalog" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analog' && echo "SHOULD BE analogue" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'analogue' && echo "SHOULD BE analog" && exit 1 || true; }
	#cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'traveling' && echo "SHOULD BE travelling" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'travelling' && echo "SHOULD BE traveling" && exit 1 || true; }
	#cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'behavior' && echo "SHOULD BE behaviour" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'behaviour' && echo "SHOULD BE behavior" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'can not' && echo "SHOULD BE cannot  see https://www.merriam-webster.com/grammar/cannot-vs-can-not-is-there-a-difference" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'modelling' && echo "SHOULD BE modeling" && exit 1 || true; }
	# Other AAS things
	#cat $(TEXFILE_BASENAME).tex | { grep --color=always --ignore-case '\\%' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\. ' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\]' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\. ' && echo "SHOULD BE i.e.," && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always --ignore-case ' `[a-zA-Z]' && echo "SHOULD BE \`\`" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v "s' " | { grep --color=always --ignore-case "[a-zA-Z]' " && echo "SHOULD BE \'\'" && exit 1 || true; }
	# super AAS-specific
	# https://journals.aas.org/manuscript-preparation/#figure_numbering
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'Fig\.' && echo "SHOULD BE Figure" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'Figs\.' && echo "SHOULD BE Figures" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'Sec\.' && echo "SHOULD BE Section" && exit 1 || true; }
	#
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'errorbar' && echo "SHOULD BE error bar" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'free-fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'free fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'free~fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	# https://journals.aas.org/aas-style-guide/
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always -e 'black body' -e 'black-body' -e 'black~body' && echo "SHOULD BE blackbody" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always -e 'gray body' -e 'gray-body' -e 'gray~body' && echo "SHOULD BE graybody" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always -e 'BL Lacs' -e 'BL~Lacs' && echo "SHOULD BE BL Lacertae objects, also BL Lac objects" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep -v '\\linewidth' | { grep --color=always 'linewidth' && echo "SHOULD BE line width" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'Milky Way Galaxy' && echo "SHOULD BE Milky Way (MW): the Milky Way" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always -e 'zero point' -e 'zero~point' && echo "SHOULD BE zero-point" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always -e 'radio loud' -e 'radio~loud' && echo "SHOULD BE radio-loud" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always -e 'radio quiet' -e 'radio~quiet' && echo "SHOULD BE radio-quiet" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always -e 'radio loudness' -e 'radio~loudness' && echo "SHOULD BE radio-loudness" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'metal poor' && echo "SHOULD BE metal-poor" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'metal rich' && echo "SHOULD BE metal-rich" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'flat fielding' && echo "SHOULD BE flat-fielding" && exit 1 || true; }
	# check that ORCIDs are uniq
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep '\\author\[' | awk -F'[' '{print $$2}' | awk -F']' '{print $$1}' | sort | uniq -d | grep --color=always '.' && echo "CHECK for non-uniq ORCID" && exit 1 || true; }
	
else
	# Nothing to do
	@echo "THIS DOES NOT LOOK LIKE AN AAS MANUSCRIPT - NOT ENFORCING US SPELLING"
	echo $(AAS_MANUSCRIPT_REQUIRING_US_SPELLING)
endif

# We want to check for a consistent use of 'gamma-ray' vs '$\gamma$-ray', but only if it's a journal paper:
# in a proposal draft we may have an ASCII-only abstract and LaTeX text body.
DO_IT_CHECK_GAMMA_RAY_MATH_MODE=no
ifeq ($(AAS_MANUSCRIPT_REQUIRING_US_SPELLING),yes)
DO_IT_CHECK_GAMMA_RAY_MATH_MODE=yes
endif
ifeq ($(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING),yes)
DO_IT_CHECK_GAMMA_RAY_MATH_MODE=yes
endif
check_gamma_ray_math_mode:
ifeq ($(DO_IT_CHECK_GAMMA_RAY_MATH_MODE),yes)
	@echo "THIS IS AN MNRAS OR AAS MANUSCRIPT"
	echo $(DO_IT_CHECK_GAMMA_RAY_MATH_MODE)
	{ cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep --quiet 'gamma-ray' && cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep --quiet '$$\\gamma$$-ray' && cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep --color=always -e 'gamma-ray' -e '$$\\gamma$$-ray' && echo "SHOULD BE USING CONSISTENTLY 'gamma-ray' or '$$\\gamma\$$-ray'" && exit 1 || true; }
else
	# Nothing to do
	@echo "THIS DOES NOT LOOK LIKE AN MNRAS OR AAS MANUSCRIPT - NOT ENFORCING MATH MODE for 'gamma-ray'"
	echo $(DO_IT_CHECK_GAMMA_RAY_MATH_MODE)
endif

check_km_s:
ifeq ($(TEST_KM_S),yes)
	# Check for km/s
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'km/s' && echo "SHOULD BE km\\,s$$^{-1}$$ ?" && exit 1 || true; }
endif

check_software_small_capitals:
ifeq ($(ANY_KNOWN_SOFTWARE_MENTIONED),yes)
ifeq ($(TEST_SOFTWARE_TEXTSC),yes)
	@failed=0; \
	for code in $(CODE_NAMES_CASE_INSENSITIVE); do \
		if cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g'| sed 's/\\citep{[^}]*}//g' | sed 's/\\cite{[^}]*}//g' | sed 's/\\citealt{[^}]*}//g' | sed 's/\\texttt{[^}]*}//g' | grep --quiet --ignore-case -e "\\b$$code\\b" ; then \
			! cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g' | sed 's/\\citep{[^}]*}//g' | sed 's/\\cite{[^}]*}//g' | sed 's/\\citealt{[^}]*}//g' | sed 's/\\texttt{[^}]*}//g' | grep --ignore-case -e "\\b$$code\\b" | grep -v -e 'textsc' -e 'scshape' -e '{\\sc ' >/dev/null && continue ; \
			failed=1; \
		fi; \
	done; \
	for code in $(CODE_NAMES_CASE_SENSITIVE); do \
		if cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g' | sed 's/\\citep{[^}]*}//g' | sed 's/\\cite{[^}]*}//g' | sed 's/\\citealt{[^}]*}//g' | sed 's/\\texttt{[^}]*}//g' | grep --quiet -e "\\b$$code\\b" ; then \
			! cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g' | sed 's/\\citep{[^}]*}//g' | sed 's/\\cite{[^}]*}//g' | sed 's/\\citealt{[^}]*}//g' | sed 's/\\texttt{[^}]*}//g' | grep -e "\\b$$code\\b" | grep -v -e 'textsc' -e 'scshape' -e '{\\sc ' >/dev/null && continue ; \
			failed=1; \
		fi; \
	done; \
	if [ $$failed -eq 0 ]; then \
		echo "All code names are properly formatted with 'textsc' or 'scshape'."; \
	else \
		echo "Checking for code names without 'textsc' or 'scshape' failed."; \
		echo "Displaying occurrences of code names:"; \
		for code in $(CODE_NAMES_CASE_INSENSITIVE); do \
    			cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g' | grep --color=always --ignore-case -e "\\b$$code\\b" ; \
		done; \
		for code in $(CODE_NAMES_CASE_SENSITIVE); do \
    			cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | sed 's/\\url{[^}]*}//g' | grep --color=always -e "\\b$$code\\b" ; \
		done; \
		echo "SHOULD BE \\textsc{CodeName}" ; \
		exit 1; \
	fi
else
	@echo "TEST_SOFTWARE_TEXTSC is not set to 'yes'. Skipping the test."
endif
else
	@echo "NO KNOWN SOFTWARE NAMES RECOGNIZED"
	@echo $(ANY_KNOWN_SOFTWARE_MENTIONED)
endif

check_swift_uvot_lowercase_filternames:
ifeq ($(IS_SWIFT_UVOT_MENTIONED),yes)
	# Check that Swift/UVOT filter names are lowercase
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'UVW1' && echo "Swift/UVOT FILTER NAMES SHOULD BE LOWECASE uvw1 ?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'UVM2' && echo "Swift/UVOT FILTER NAMES SHOULD BE LOWECASE uvm2 ?" && exit 1 || true; }
	cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | { grep --color=always 'UVW2' && echo "Swift/UVOT FILTER NAMES SHOULD BE LOWECASE uvw2 ?" && exit 1 || true; }
else
	# Nothing to do
	@echo "NO MENTION OF SWIFT UVOT"
	echo $(IS_SWIFT_UVOT_MENTIONED)
endif

check_consistent_unbreakable_space_size_UT:
	{ cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet '~UT' && cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet '\\\,UT' && cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --color=always -e '~UT' -e '\\\,UT' && echo "SHOULD BE USING CONSISTENTLY '~UT' or '\\,UT" && exit 1 || true; }

check_consistent_Halpha_Hbeta:
	#cat *.tex | cut -f1 -d"%" | grep --quiet -e 'H\$$_\\beta\$$' && exit 1
	{ cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet -e 'H\$$_\\beta\$$' -e 'H\$$_\\alpha\$$' && cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet -e 'H\$$\\beta\$$' -e 'H\$$\\alpha\$$' && cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --color=always  -e 'H\$$_\\beta\$$' -e 'H\$$_\\alpha\$$'  -e 'H\$$\\beta\$$' -e 'H\$$\\alpha\$$' && echo "SHOULD BE USING CONSISTENTLY 'H$$\\beta\$$' or 'H\$$_\\beta\$$' (with the underscore)" && exit 1 || true; }

check_consistent_multiwavelength:
	{ cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet -e 'H\$$_\\beta\$$' -e 'H\$$_\\alpha\$$' && cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --quiet 'multi-wavelength' && cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d"%" | grep --color=always  'multiwavelength' && echo "SHOULD BE USING CONSISTENTLY 'multi-wavelength' or 'multiwavelength'" && exit 1 || true; }


check_filenames_good_for_arXiv:
	# Check if all filenames in the current directory contain only characters that are good for arXiv
	# as listed at https://info.arxiv.org/help/submit/index.html#files
	{ for FILENAME in * ;do if [[ "$$FILENAME" =~ ^[0-9A-Za-z_\\.\\,\-\\=\\+]+$$ ]]; then echo "The filename '$$FILENAME' looks good"; else echo "The filename '$$FILENAME' has characters not good for arXiv"; fi ;done | grep --color=always 'characters not good for arXiv' && exit 1 || true; }



$(TEXFILE_BASENAME).pdf: $(TEXFILE_BASENAME).tex
ifeq ($(PDFTEX),yes)
	# pdflatex
	@echo "YES PDF"
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	@echo "YES BibTeX"
	echo $(BIBTEX)
	# This works with .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex || echo "Looks like texcount is not installed - Makefile can't count words in the LaTeX file"
endif
else
	@echo "NO BibTeX"
	echo $(BIBTEX)
	# No BibTeX, .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex || echo "Looks like texcount is not installed - Makefile can't count words in the LaTeX file"
endif
endif

else
	# latex
	@echo "NO PDF  "
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	@echo "YES BibTeX"
	echo $(BIBTEX)
	# BibTeX and .eps figures (the right way)
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && latex $(TEXFILE_BASENAME).tex && { latex $(TEXFILE_BASENAME).tex 2>&1 | grep --color=always 'undefined on input line' && exit 1 || true; } && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex || echo "Looks like texcount is not installed - Makefile can't count words in the LaTeX file"
endif
else
	@echo "NO BibTeX"
	echo $(BIBTEX)	
	# This works with .eps figures or when \usepackage[demo]{graphicx} is activated
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps 
ifeq ($(COUNT_NUMBER_OF_CHARACTERS_WITH_TEXCOUNT),yes)
	texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex || echo "Looks like texcount is not installed - Makefile can't count words in the LaTeX file"
endif
endif

endif


check_for_bonus_figures: $(TEXFILE_BASENAME).tex
	{ for i in *eps *png *jpg ;do if [ ! -f $$i ];then continue ;fi ; cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d'%' | grep --quiet "$$i" && continue ; echo "WARNING: a bonus figure not included in the TeX source: $$i" ;done ; echo " " ; }  && { cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d'%' | grep 'label{fig:' | awk -F'label{' '{print $$2}' | awk -F'}' '{print $$1}' | while read LABELLED_FIGURE ; do cat $(ALL_TEXFILES_FOR_GRAMMAR_CHECK) | cut -f1 -d'%' | grep --quiet "ref{$$LABELLED_FIGURE}" && continue ; echo "WARNING: a figure not referenced in the main text: $$LABELLED_FIGURE" ;done ; echo " " ; }


produce_balck_and_white_copy_of_the_pdf: $(TEXFILE_BASENAME).pdf
ifeq ($(PRODUCE_BLACK_AND_WHITE_COPY_OF_THE_PDF_TO_CHECK_HOW_IT_LOOKS),yes)
	@echo "Producing a black and white (grayscale) copy of "$(TEXFILE_BASENAME).pdf
	# -dCompressPages=false is used to speed up compilation by a second
	gs -sOutputFile=$(TEXFILE_BASENAME)_grayscale.pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompressPages=false -dNOPAUSE -dBATCH $(TEXFILE_BASENAME).pdf
	@echo "The grayscale copy of the document is written to "$(TEXFILE_BASENAME)_grayscale.pdf
endif



display_compiled_pdf: $(TEXFILE_BASENAME).pdf
	@echo "The document is successfully compiled: "$(TEXFILE_BASENAME).pdf
ifeq ($(LAUNCH_PDF_VIEWER_TO_DISPLAY_COMPILED_PAPER),yes)
	@echo "Trying to find a PDF viewer to display "$(TEXFILE_BASENAME).pdf
	okular $(TEXFILE_BASENAME).pdf || evince $(TEXFILE_BASENAME).pdf || xpdf $(TEXFILE_BASENAME).pdf || mupdf $(TEXFILE_BASENAME).pdf || open -a Preview $(TEXFILE_BASENAME).pdf || open -a "Adobe Acrobat Reader" $(TEXFILE_BASENAME).pdf || open -a Skim $(TEXFILE_BASENAME).pdf || firefox $(TEXFILE_BASENAME).pdf || /Applications/Firefox.app/Contents/MacOS/firefox $(TEXFILE_BASENAME).pdf || google-chrome $(TEXFILE_BASENAME).pdf || google-chrome-stable $(TEXFILE_BASENAME).pdf || chromium $(TEXFILE_BASENAME).pdf || echo "Sorry, the Makefile can't find a PDF viewer to automatically display the compiled "$(TEXFILE_BASENAME).pdf
endif


==> README <==
============================================================

   gensymb – Generic symbols for both text and math mode

============================================================
Walter Schmidt

Keiran  Harcombe
kjh@harcombe.net
  
This LaTeX package provides generic commands
\degree, \celsius, \perthousand, \micro and \ohm, which
work both in text and math mode.  The package should
co-operate flawlessly with the well-known units.sty.
Various means are provided to fake the symbols or take
them from external symbol fonts, if they are not available
in the default fonts used in the document.  The package
makes optionally use of upgreek.sty.

The style files can be unpacked by running the particular
installation script (.ins) through LaTeX.  The files will 
be created immediately in the appropriate TDS directory
tex/latex/was, if this directory exists and the DOCSTRIP
tool is properly configured -- otherwise they are written
into the current directory.

The documentation of a package can be generated by running
the particular .dtx file through LaTeX.

==finis

